Explicit Quantum Circuits for Block Encodings of Certain Sparse Matrices

Many standard linear algebra problems can be solved on a quantum computer by using recently developed quantum linear algebra algorithms that make use of block encodings and quantum eigenvalue/singular value transformations. A block encoding embeds a properly scaled matrix of interest A in a larger unitary transformation U that can be decomposed into a product of simpler unitaries and implemented efficiently on a quantum computer. Although quantum algorithms can potentially achieve exponential speedup in solving linear algebra problems compared to the best classical algorithm, such gain in efficiency ultimately hinges on our ability to construct an efficient quantum circuit for the block encoding of A, which is difficult in general, and not trivial even for well-structured sparse matrices. In this paper, we give a few examples on how efficient quantum circuits can be explicitly constructed for some well-structured sparse matrices, and discuss a few strategies used in these constructions. We also provide implementations of these quantum circuits in MATLAB.

==> shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{amsfonts}
\usepackage{mathtools}
\usepackage{mymath}
\usepackage{braket}
\usepackage{myqcircuit}
\usepackage{graphicx}
\usepackage[caption=false]{subfig}
\usepackage{listings}
\usepackage{comment}
\usepackage[edges]{forest}
\usepackage{cite}
\usepackage{placeins}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
%\newsiamremark{remark}{Remark}
%\newsiamremark{hypothesis}{Hypothesis}
%\crefname{hypothesis}{Hypothesis}{Hypotheses}
%\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Quantum Circuits for Block Encodings}{D. Camps, L. Lin, R. Van Beeumen, and C. Yang}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Explicit Quantum Circuits for Block Encodings of Certain Sparse Matrices}
%\thanks{Submitted to the editors DATE.
%\funding{This work was funded by the Fog Research Institute under contract no.~FRI-454.}}}

% Authors: full names plus addresses.
\author{Daan Camps\thanks{%
  Applied Mathematics and Computational Research Division,
  Lawrence Berkeley National Laboratory, Berkeley, CA
  (\email{dcamps@lbl.gov}, \email{rvanbeeumen@lbl.gov}, \email{cyang@lbl.gov}).}
\and Lin Lin\thanks{%
  Department of Mathematics and Challenge Institute of Quantum Computation, University of California, Berkeley, CA and
  Applied Mathematics and Computational Research Division,
  Lawrence Berkeley National Laboratory, Berkeley, CA
  (\email{linlin@math.berkeley.edu}).}
\and Roel Van Beeumen\footnotemark[1]
\and Chao Yang\footnotemark[1]}

\DeclareMathOperator{\swap}{\textsc{Swap}}
\DeclareMathOperator{\refl}{\textsc{Ref}}
\newcommand{\DC}[1]{{\color{teal}~\texttt{DC: #1}}}
\newcommand{\CY}[1]{{\color{red}~\texttt{CY: #1}}}
\newcommand{\rvb}[1]{{\color{orange}~\texttt{RVB: #1}}}
\newcommand{\LL}[1]{\textcolor{brown}{[LL:#1 ]}}

\newcommand{\rev}[1]{{#1}}
\newcommand{\revii}[1]{\textcolor{blue}{#1}}

\newcommand{\Us}[1]{U^{(#1)}}
\newcommand{\hlfpi}{\frac{\pi}{2}}

%% LL macros
\newcommand{\opr}[1]{\ensuremath{\operatorname{#1}}}
\newcommand{\BE}{\operatorname{BE}}
\newcommand{\HBE}{\operatorname{HBE}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\Or}{\mathcal{O}}
\newcommand{\wt}[1]{\widetilde{#1}}

% ---- Tikz ------------------------------------------------------------------ %
%\ifnum\externalizetikz=2
%  \usepackage{tikzexternal}
%  \tikzexternalize
%  \tikzsetexternalprefix{fig/}
%\else
  \usepackage{tikz}
  \usepackage{pgfplots}
  \usetikzlibrary{calc}
  \usetikzlibrary{positioning}
  \usetikzlibrary{plotmarks}
  \usetikzlibrary{automata,arrows,matrix,quotes}
  \pgfplotsset{
    compat=newest,
    table/header=false,
    tick label style={font=\scriptsize},
    label style={font=\scriptsize},
    legend style={font=\scriptsize},
    legend cell align=left,
    colormap={parula}{
      rgb255=(53,42,135)
      rgb255=(15,92,221)
      rgb255=(18,125,216)
      rgb255=(7,156,207)
      rgb255=(21,177,180)
      rgb255=(89,189,140)
      rgb255=(165,190,107)
      rgb255=(225,185,82)
      rgb255=(252,206,46)
      rgb255=(249,251,14)
    }
  }
  \pgfplotsset{
    myColOne/.style={myblue},
    myColTwo/.style={myred},
    myColThr/.style={myorange},
    myColFou/.style={mypurple},
    myColFiv/.style={mygreen},
    myColSix/.style={mylightblue},
    myColSev/.style={mydarkred}
  }
%  \ifnum\externalizetikz=1
%    \usepgfplotslibrary{external}
%    \tikzexternalize[prefix=fig/]
%  \fi
%\fi
\newcommand{\figname}[1]{\tikzsetnextfilename{#1}}
\newcommand{\fignames}[1]{\tikzsetfigurename{#1}}
\newcommand{\datfile}[1]{fig/#1.dat}
% ---------------------------------------------------------------------------- %

%%% Local Variables:
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End:

